Two case studies on implementing best practices for Software Process Improvement

Software Process Improvement requires significant effort related not only to the identification of relevant issues and providing an adequate response to them but also to the implementation and adoption of the changes. Best practices provide recommendations to software teams on how to address the identified objectives in practice, based on aggregated experience and knowledge. In the paper, we present the GEANT experience and observations from the process of adopting the best practices and present the setting we have been using.

==> monitoring.tex <==
\section{}
\label{sec:monitoring}

%NEW
%description of the approach to monitoring:
%1. Principles and assumptions
% - non-intrusive, low-effort
% - avoiding evaluation
% - bidirectional feedback-driven: the approach it adjusted, based on the results of evaluation
% simplicity and intuitiveness over precision
%2. Process of monitoring
% - methods: interviews, periodic updates
% stakeholders: teams + SwM team
%2. Tool support
% description of the plugin
%3. Limitationshttps://www.overleaf.com/project/60587a3ad1bff038588bbf4c
% insufficient data

% what is monitoring, what it includes: adoption, reach of change, consolidation + promotion

The process of implementing best practices and transferring them between various teams is organized into four iteratively repeated phases:
\begin{enumerate}
    \item Understanding the critical and important processes and practices in each team's work (by interviewing the team members),
    \item Reaching the agreement with the team concerning the implementation of SPI recommendations, making necessary adaptations and adjustments,
    \item Monitoring the adoption process and refining the approach,
    \item Evaluating the results, providing feedback and formulating new or updating the existing SPI-related recommendations.
\end{enumerate}

In the process, we intentionally avoid using the term "evaluation", which is associated with feedback not exclusively related to process improvement, but also the inevitable comparison of teams. Initial attempts to include an element of assessment was found to be too offensive by many teams and significantly hampered their motivation to participate in the SPI program. As a result, we decided to re-focus our attention on activities directly linked with process optimization.

In the following subsections, we provide more insights into key aspects of the process.


%)---
%ensuring that the is to establish an understanding of the needs and maturity of the G\'{E}ANT teams. On top of that, the feedback from the monitoring process is collected and analysed and used to validate that the right topics are being pursued, questions asked and items monitored. The collected information will help in refining the practices and adding new ones on the base of collected and analysed needs and current practices of software teams.
%)---

\subsection{Adaptation and operationalization of best practices}
\label{ssec:adaptation}
Adaptation is an indispensable step in the SPI process in the G\'{E}ANT context. Best practices that have been identified and documented do not deliver directly executable instructions, but directional recommendations at a high level of abstractness. This was a conscious decision, given the diversity of the solutions that addressed each objective in SMM, which could not be embraced by a single, universal practice. Consequently, the recommendations included in CBPs need to be customized and adapted to the local context of the implementing team. In practice, this happens in a sequence of interactions between SwM and the software team, with the following outline:
\begin{enumerate}
    \item Presentation of the catalogue of CBPs to the software team, with a concluding discussion;
    \item Selection of the practices, for which there exists the largest room for improvement;
    \item Presentation of the current status of the given objective;
    \item Adaptation and operationalization of the best practice, with an objective to address the specific context of the team;
    \item Defining preliminary metrics and parameters for monitoring the adoption process.
\end{enumerate}

In this process, two items deserve a comment. First, operationalization of the practice mostly concerns the translation of the generic recommendations of the practice into actionable statements that encompass the specific context of the team, its tools and procedures. Additionally, sometimes a specific practice also needs to be extended or narrowed, as some elements of it are out of scope in the team's context. As a result, the team can elaborate its own version of the practices, as long as their objectives are properly addressed.

The process of adoption needs to be controlled and managed based on quantitative values. Since \emph{modus operandi} varies among teams, the monitoring metrics are frequently identified in each case separately. As a side effect, due to the differences in metrics and parameters, it is virtually impossible to perform a cross-project comparative evaluation. However, we need to outline that the evaluating aspect of best practices adoption is not the top priority. 
At this stage, we only make a preliminary identification of the metrics, while they are fixed, tuned and calibrated in the next step. 

\subsection{Monitoring}
\label{ssec:monitoring}

Monitoring is another step in the deployment step that allows for controlling the process, collecting feedback and taking necessary corrective actions. It fosters the adoption of best practices, contributes to increasing the outreach of change, supports the consolidation of achieved results and is also a promotional tool that encourages the implementation of similar ventures in other teams.

% monitoring is not evaluation
The monitoring activity needs to be backed and guided by data, either quantitative or qualitative. However, since the initial status of software teams is diverse, and their specific needs and methods differ and are subject to subjective assessment and interpretation, it is very difficult to provide a single measure that would be universally applicable. 
The measurement can be also used as a feedback tool that will allow not only to evaluate the outcomes but also to validate and adjust them. 
%EXAMPLE

\subsection{Tool support}
\label{ssec:tool}

To effectively support the monitoring process, adequate instrumentation is needed. The process of monitoring requires collecting  feedback data for tuning and taking corrective actions regularly. The feedback loop is similar to the one used for agile software development with two differences: it should require a lower level of engagement from the team (as the SPI process is usually only accompanying the primary activity), and it spans over a longer time, as it is not related to direct results of software development, but to the changes in development methods. %Therefore, changes that are detected and assessed through this dialogue can typically be measured and recorded monthly. 
%In addition to established and monitored contextualized mappings of general recommendations and concerns for the specific situation, that are the primary inputs for these interviews, it is also useful to monitor and discuss the related measures that quantify workflow results, such as source code metrics, incident frequency, number of served requests, user satisfaction, use of advanced or new features, responsiveness or level of user participation, user retention and the like. These metrics should not be interpreted as immediate or exclusive indicators of software team performance in the observed area, but as indicators that represent the inputs for the evaluation and as evidence illustrating the changes that have occurred while the changes in the approach have been made. Metrics that directly track the process and not just some characteristics of its outputs, are the most convenient as they reflect the organization and the level of optimization of the process because only an apprehended and structured process can be measured and only a measured process can be improved.

To properly support the monitoring of the adoption of CBPs, we added a data collection and visualization plugin into the G\'{E}ANT Software Catalogue (GSC). GSC is a system that collects and manages information about all software projects in G\'{E}ANT. It is available to the SwM team, software teams and other stakeholders so that it provides continual access to all measurements and data. GSC regularly collects information from various components of the toolchain that  may be useful for this purpose, e.g., issue tracker, directory service or code repositories. 

The CBPs plugin relies on the data available in GSC but it also allows for defining  manually maintained metrics related to the adoption of CBPs in specific projects. In particular, the tool allows for defining arbitrary metrics that correspond to the process and entering the measurements by authorized stakeholders from G\'{E}ANT. For each metric we defined an ordinal scale of values; in many cases, a five-point Likert scale is used, which provides some uniformity across teams and practices. Stakeholders record changes in the monitored quantities and can observe the changes in the reported values.

In addition to the main metrics for individual best practices, it is also useful to monitor and discuss the related measures that quantify workflow results, such as source code metrics, incident frequency, number of served requests, user satisfaction, responsiveness or level of user participation, user retention and the like. They are also supported by the CBPs plugin and are used as customisable supporting and indicative metrics for individual best practices that provide evidence for the best practices or can be used to help in assisting its current status. These metrics are currently also manually collected, but in the future could be linked to the information that GSC already regularly collects from some of the tools it is integrated with.

Although all these quantities are currently monitored manually, in the future they could be extracted and analysed by an external tool. However, we do not expect that the monitoring will ever be fully automated, as the final appraisal of practice is highly context-dependent. %However, as the number of tracked metrics will never exceed just a few, it is not a major obstacle.

==> studyA.tex <==
\subsection{Project A}
\label{sec:projectA}

% Context of two case studies, presenting the background, staff, objectives

% context of the project (history, objectives, staff, liveness)
% history of engagement with CBP
% identified areas and applied best practices
% AUTHOR: BM + IG

In our SPI process we were guided by the following steps:

\begin{enumerate}
\item Identify and scope the area of improvement in the context of the G\'{E}ANT CBPs.
\item Agree on an approach for the implementation of process improvements.
\item Observe progress and refine the approach.
\item Conclude the process and evaluate results.
\item Consider a success story. !!!I HOPE THAT THE STYLE GUIDE ALLOWS SENTENCES IN BULLETS - WAS IN SMALL LETTERS AND WITHOUT PERIODS!!!!
\end{enumerate}

%MW - new paragraph - BW - please approve
We have defined an unobtrusive mechanism for continuous collection of software teams' practices performance and to indicate further needs in this area. This mechanism is implemented as a feature of the G\'{E}ANT Software Catalogue (https://sc.geant.org). 
% screenshot from SC can be placed here - see sc.png

A member of the SMT can report directly in the Software Catalogue on the evaluation of a specific practice. Each evaluation is described by several attributes, such as a timestamp or a scale. Values on the scale show how well a given team has adopted the practices. The values can also be supplemented by a comment, which gives a more thorough picture of the process at the moment. Having the evaluation recorded, a team member can get an insight into practices implemented by the team or see the progress in practices implementation within a specific period.

!!! THE ABOVE TEXT APPLIES TO BOTH A AND B !!!

\subsection{Overview of the project}

We worked in close cooperation with a development team for the subject project. The team works on a software platform WiFiMon used for the assessment and monitoring of the WiFi performance and user experience in campus areas. This is done by engaging end-user devices in short anonymised data exchanges at the time of the WiFi connection establishment to gather multiple network performance statistics. The architecture comprises of a server side for measurement, data collection and GUI with monitoring modules. 
The team provides the software as a product for organisations interested in the project. In addition to the product support on a dedicated channel, the team maintains a live demo environment for the data collection and GUI systems.

\subsection{Identified needs and expectations}

In the collaboration process, we tried to understand and then agree upon an area of improvement from a broad collection of established best practices found vital for the development environment of the G\'{E}ANT project. The common best practice agreed for improvement was "BP-E.4: Define a procedure for deploying changes to running services" and an improvement plan with project-related objectives was created in order to follow the development of the best practice adoption. The objectives were prescribed according to the recommendations defined in the BP document.

\subsection{Practices selected for implementation}
The BP-E.4 practice is focused on the process of implementing changes to services in operation, which requires a good understanding of the dependencies of the running system, the risks associated with the management of operational data and the tight coordination between the different operational teams, which provide supporting generic services for example, but not limited to, network connectivity or operating system management in an attempt to minimise the running service downtime.  

Following the established SPI process, a first-level evaluation was prepared based on the agreed objectives to serve as a base for our progress evaluation process.
\subsection{Results}
The WiFiMon team built the internal service to track the versions of the software ran by customers and to identify those who are actively using WiFiMon. In the process, they also formalised the internal release management and tagging and they are collecting the version checks (automated or by users) data from the active instances.

In the outcome, the WifiMon team improved and is now running an ordered, disciplined and data-informed process related to the version management, tracking the product usage and associating versions with specific customers and their issues, needs and questions.

\begin{table}[]
\label{tab:projectAmetrics}
\caption{Results of evaluation for the BP-E.4 best practice in Project A}
\centering
\begin{tabular}{lrrr}
\toprule
Metric  & \multicolumn{3}{c}{Month} \\
        & 1         & 5         & 15\\ 
\midrule
General evaluation & 3/7 & 6/7 & 7/7\\
\midrule
Orderly collection of new feature requests
& YES            & YES               & YES              \\
Procedure for determining what features are to be added to the new release
& YES             & YES              & YES              \\
Predefined release schedule
& YES             & YES              & YES              \\
\midrule
Communication channel for informing users about updates                                                            & NO             & YES              & YES              \\
Mechanism for performing or nudging updates                                                            & NO             & YES              & YES              \\
Tool or method for collecting the data about used versions and updates                                                            & NO             & YES              & YES              \\
Collected data is used in analysis and planning                                                            & NO             & NO              & YES              \\
\midrule
\bottomrule
\end{tabular}
\end{table}

These changes were the result of the additions to delivery, deployment, monitoring, user support, and release planning that were articulated during the joint sessions of SwM and Project A teams. These additions were expressed as clear and straightforward software features, utilities and procedural changes, which enabled the developers and supporters to adopt them as practical and valuable modifications, easily implement the needed elements and get concrete and immediate improvements. All devised and agreed interventions have been implemented and data is collected as a part of the monitoring process and periodically analysed. 

An internal procedure for deploying, validating or reverting the changes was established and applied. Information about the new releases and summaries of contained changes are timely distributed to registered users. Furthermore, the project team has established the process of collecting records that describe and track features and issues reported by users and testers. The instances of the software update automatically or inform the user about available updates and assist in their download and installation. The team also developed a method for collecting the data about used the usage and versions of WiFiMon instances and the rollout of updates. The tracked parameters are the numbers of active instances and downloads and the percentage of users running the latest version. Data about changes, their availability, deployments, active instances and related user behaviours and response times are used in analysis and planning to enhance release management, deployment process or communication with users. If new problems or opportunities for improvement are identified, they will be used to further refine the team's procedures, software tools and metrics, and also the related best practices.

%During the monitoring period, these statistics were collected and tracked. 

%At the last checkpoint, we observed the peak of active instances during the second quarter of the monitoring period. The number of downloads also slightly increased, as well as the percentage of users running the latest version. There have been some test instances installed during this period, which were not supposed to be used in the long run.


%OLD

%One of the key goals for analysis is to perform comparative ranking and clustering of topics based on their rating by participants of the survey. In the future, we plan to focus primarily on the areas where the greatest gains could be accrued in terms of practices improvements. The data collected so far significantly contributed to the selection of topics that should be promoted, worked on and supported through the improvement incentives.

%One of the goals for analysis was to identify the areas that deserve most attention and effort. The data collected so helped in the selection of topics that should be promoted, worked on and supported through the improvement incentives. Below, we provide comments on them:
 
%\begin{itemize}
%    \item The first candidate areas and specific goals are those for with the greatest diversity in the responses to related questions in the conducted survey in terms of satisfaction and expressed knowledge of associated practices. These are the topics where the benefit could be achieved with the least effort and by relying on the available internal expertise and through the harmonisation of knowledge and practices across teams. Although needs may vary from team to team, this harmonisation would contribute to mobility between teams due to the reconciliation of internal standards and, indirectly, external expectations. 

%    \item First, we focused on the areas in which the declared knowledge and satisfaction of the software teams was the most diversified. For those items, we can rely on the immediately available internal expertise of some teams, which reduces the effort needed for process improvement. Such harmonisation of processes among teams could additionally strengthen their collaboration.

%    \item Another issue refers to areas 
    %where the reaction is needed are those 
%    for which the survey scores were generally low or mediocre. These can be interpreted two-fold: either (1) the survey has identified a relevant topic that has been underestimated and has not been covered adequately, or (2) the topic is considered irrelevant by developers. To determine the actual status of these topics, teams and their leaders should be consulted. For that reason, it is useful at this point to establish a regular mechanism for collecting feedback from software teams. 
    %If a topic is to be incorporated, it may be necessary to change the current context, reformulate or change the strategic goals or enhance communication of existing ones. 
%    The apparent difficulty associated with these topics is the insufficient internal experience, so it may be necessary to look for external expertise and support to achieve the expected improvements.%, as well as to attain a wide mobilisation, as all teams need to improve in these areas.

 %   \item The third group of interest includes the areas with uniformly high marks. Here, we can expect relatively small improvements, even if the collected data is not completely accurate. High grades given by all teams may indicate that the reached level cannot or should not be further improved.%, and hint the lack the willingness and incentive to improve things further, as everyone thinks that everything in that area is good. Of course, senior-level management can propose or request improvements even in the areas where grades are consistently high.

%    \item In the third group are the areas where the marks are uniformly high. Here, the smallest gains can be expected, even if the obtained image is not completely accurate. Uniform high grades are an indication of the shared view that the reached level cannot or should not be raised further, and hint the lack the willingness and incentive to improve things further, as everyone thinks that everything in that area is good. Of course, senior-level management can propose or request improvements even in the areas where grades are consistently high.

% \end{itemize} #IG# this one was creating an error, so added space between \ end

%MW - I don't quite follow this part - it contains valuable recommendation, like for example the one to consult with management etc. But I think such recommendations are rather a part of the internal documents than a public paper?

%BM - this is generic of the proposed process and logic, with indications of convenient inflection points where  the higher management could intervene or be consulted. So I returned this to the paper. But wording could be changed or some additional explanations could be given if you feel uneasy with this...

%At this point, it is convenient to consult with the management that directs project activities within which software development is performed. Specifically, they can correct and further streamline the expert views articulated through the GSMM topics and the questionnaire used in the survey, as well as interpretations of responses. The convenience of this moment is additionally reflected in the availability of the thematic structure established by the GSMM team, data about teams' opinions about offered topics, as well as first-level filtering of topics, as described above. This gives the managers a set of choices and arguments that can help them make informed and optimal decisions. From the point of the enhancement of software engineering across G\'{E}ANT teams, this also contributes to strengthening the mandate to implement improvements and further engage software development teams.


%The instruments established to collect feedback from software teams should not be used just to address the dilemmas related to the selection of improvement areas. They could be also applied to get a response about the ongoing improvement initiatives and track the metrics that are relevant for the implementation of the GSMM. However, conducting extensive interview-based surveys, like the one described in Section~\ref{sec:process}, requires significant effort; at next stages, they could be supported with simpler and frequently run online questionnaires that focus on the key elements. %and include fewer questions and closed answer lists.
%These questions should be used to determine the needs and interests for potential new topics, track changes in indicators associated with already approved topics and even suggest and assess new indicators.

%Optionally, this approach could be taken even further by associating the indicators with maturity levels. Maturity is assessed against key capability and practice characteristics linked with the selected target areas at each level of the model. Maturity levels are typically established using a five-point Likert scale where the higher the level, the higher is the level of maturity. These progressive levels guide the planning and development of roadmaps. 
%It is good to use the same scale and general descriptions of levels as in other maturity models since this facilitates mixing or aligning of several related but distinct maturity models. With this, it is possible to determine the maturity level against a set of predefined criteria and to develop corresponding self-evaluation or certification tools. 
%As the subject of evaluation may demonstrate different maturity levels within individual areas and for different indicators, typically the lowest one found is used to determine the overall maturity. 
%Currently, there is no need for G\'{E}ANT to develop such a far-reaching maturity model. A future move in this direction would require reaching beyond G\'{E}ANT into an even larger base of software teams to capture the indicators and link their values to maturity levels.
%as this is the only way to justify the effort and produce stable and non-disputable indicators and levels. 
%Given the number of potential indicators and certain subjectivity in associating them with maturity levels, it is necessary to draw from the opinions and attitudes of a larger community to get non-disputable criteria. 
%The capture from a much larger group of actors and sources would also ensure better coverage of the diverse and heterogeneous software governance ecosystem. 
%Although other related standardisation processes and schemes and maturity models could additionally support this development, it is crucial to establish and employ a simple, inclusive and quality process in which the indicators and levels are produced and challenged. Again, a series of simple and low-effort online surveys could be used to iteratively establish and maintain the set of used indicators and maturity criteria.

%Observations/Results:
%\begin{itemize}
%    \item There is diversity in meeting the goals in G\'{E}ANT across teams and in various areas
%    \item a maturity model should capture the key areas, addressing the context, constraints and opportunities
%    \item objectives are not enough; they should be accompanied by directing guidelines; we call them ``best practices''
%    \item Best practices provide ``soft'' guidance on how to meet the specified goals; they should be derived from the goals they address
%    \item Best practices need to be structured (outline their resemblance to design patterns!)
%    \item Best practices should instruct 'what', rather than 'how'. How may be too specific. That activates the teams and ensures they adapt the BPs to their environment
%    \item Their level of details should be above procedures should be more general than procedures, but also address the context and constraints of the organisations
%\end{itemize}

==> studyB.tex <==
\section{Project B}
\label{sec:projectB}

% same as Project A
% AUTHOR: BW

\subsection{Overview of the project}
Project B is an internal online catalogue that includes comprehensive information about software projects developed and maintained in G\'{E}ANT. Unlike other similar systems, it does not rely on data entered manually by operators or users, but rather actively looks for changes in the available data sources (such as software development tools) and updates its internal databases. The offered data is diverse; for example, it displays the description and current status of the project, its current and previous staff, external organisations involved in it, but also development-related activity in the code repository, quality-related reports, the employed technology stack, and also some specific SPI-related information. In addition, the project is also endowed with a full-text search engine, which helps the users in finding the relevant piece of information. From the functional point of view, Project B is a central informational hub with comprehensive data about the projects.

\subsection{Identified needs and expectations}
Project B is managed from the beginning by a consistent team of developers, with a clear vision of the product. As a result, several processes and software engineering practices and properly implemented, addressed and aligned. However, the team decided to participate in the best practice assessment with an objective to identify deviations, quality hotspots and opportunities for improvement.

Specifically, the team decided to focus on two specific goals: the management of stakeholders, and the elements of quality assurance. Both of them have been partially implemented by achieving and documenting some objectives, while some aspects have not been addressed yet. The implementation of best practices provided a good opportunity for improving the status vis-à-vis these goals.

\subsection{Practices selected for implementation}
A number of meetings and interviews allowed for the identification of two best practices that correspond to the objectives set by the team. Their current statuses have been investigated, scrutinised and summarised, and then the results would have been implemented by the Project B team.
\begin{itemize}
\item BP-A.1: Identify an initial group of stakeholders and iteratively refine it.
\item BP-C.2: Identify relevant quality characteristics and test conditions, and provide verification criteria for them.
\end{itemize}

The BP-A.1 practice is focused on having a closely engaged group of stakeholders, who would and could help in collecting requirements and user needs. The stakeholders could also contribute to other areas of the project, e.g., identification of risks (BP-C.1) or definition of user acceptance tests (BP-C.4).
In Project B, this aspect has been addressed by creating and maintaining a list of stakeholders. The list is managed by the team leader and periodically reviewed by including new people, removing inactive ones or updating declarative info, contacts and similar data. Each communication targeted to the stakeholders is also noted to monitor the frequency of meetings as well.
The part of the practice that has not been implemented concerns the prioritisation of stakeholders. For now, all of them are considered equally involved in the project, which does not reflect the needs. The recommended solution would be to identify a group of key stakeholders who would be consulted regularly, and the remaining ones, who would be only informed about the changes and the progress. 

The BP-C.3 practice is directly linked with the approach to quality assurance in the project. The initial outline of testing activities has been defined at the beginning of the project, and then it has been updated, re-analysed and operationalised in the project.

The Project B team employs three levels of tests: unit tests, implemented and executed by each programmer, system tests based on exploration, and user A/B tests. Presently, the missing part includes user acceptance tests (UAT) for the application, and that has been selected as an immediate objective for the best practice implementation.

\subsection{Results}

Implementation of those best practices has been monitored with a set of metrics that were produced by adapting the predefined ones for that practice. The results of two evaluations are reported in Tables~\ref{tab:projectBmetricsA1} and \ref{tab:projectBmetricsC2}. They are rather indicative than conclusive and provide some information on how the assessment is being made.

\begin{table}[]
\caption{Results of evaluation for the BP-A.1 best practice in Project B}
\centering
\begin{tabular}{lrr}
\toprule
Metric  & \multicolumn{2}{c}{Date of assessment} \\
        & 26/11         & 22/12         \\ 
\midrule
General evaluation & 4/5 & 5/5 \\
\midrule
Are stakeholders prioritised?                                                            & NO             & YES               \\
Is the list of stakeholders updated on a regular basis?                                 & YES            & YES               \\
Are the stakeholders' needs tracked to requirements?                                    & YES             & YES               \\ 
\midrule
Number of identified and contacted stakeholders & 14  & 14  \\
Time since contact with a stakeholder (about requirements) {[}days{]} 
    & N/A               & N/A               \\ 
Time since contact with a stakeholder (about UAT) {[}days{]}          
    & N/A               & N/A               \\ 
\bottomrule
\end{tabular}
\label{tab:projectBmetricsA1}
\end{table}

There are three simple Boolean metrics. They directly refer to facts, not evaluation, which makes them the most objective. However, they also carry limited information, which can be supplemented with a description. In that case, the assessor provided no remarks.
Additionally, there are also three regular metrics. They capture the number of stakeholders that have been identified by the team, and the time since contacting any stakeholder with respect to requirements and UATs, which reflects the activity in communication with them. The two time-related metrics are not being monitored, as the data has not been collected so far. The team also decided that they are not relevant in that case.

The first assessment found that a relatively large group of stakeholders is managed in the same way, which did not properly reflect the real needs. The SwM and Project B teams have decided to refine the list of stakeholders to identify key stakeholders and involve them more closely in the project. A list of key stakeholders was created, which was appreciated during the second assessment. 

\begin{table}[]
\caption{Results of evaluation for the BP-C.2 best practice in Project B}
\centering
\begin{tabular}{lrr}
\toprule
Metric  & \multicolumn{2}{c}{Date of assessment} \\
        & DD/MM         & DD/MM         \\ 
\midrule
General evaluation & X/5 & X/5 \\
\midrule
Are stakeholders prioritised?                                                            & NO             & YES               \\
Is the list of stakeholders updated regularly?                                 & YES            & YES               \\
Are the stakeholders' needs tracked to requirements?                                    & YES             & YES               \\ 
\midrule
Number of identified and contacted stakeholders & 14  & 14  \\
Time since contact with a stakeholder (about requirements) {[}days{]} 
    & N/A               & N/A               \\ 
Time since contact with a stakeholder (about UAT) {[}days{]}          
    & N/A               & N/A               \\ 
\bottomrule
\end{tabular}
\label{tab:projectBmetricsC2}
\end{table}

Currently, all recommendations for the practice have been implemented, and now it needs to be only monitored. If new opportunities for improvement would be identified, then they could result in defining another, more refined best practice.




==> test.tex <==
\section{Background}
\label{sec:background}

% Refer to the previous work on SPI in GEANT (SMM, CBP), recall the structure of GEANT, shortly present the CBP framework and its relation to SMM
% We also need to refer to the three-level structure of CBP framework: target domain, specific practices (with recommendations and risks), and metrics allowing for monitoring and tracking
%IMportant: present the GN structure for SPI: the role of SwM, the constraints for SDTs etc.
% AUTHOR: MW + BW


G\'{E}ANT is a large pan-European project that initially originated from networking, but currently it has become a leader in delivering innovative solutions for research and academia, by embracing complex software components and systems and defining services atop of the network. As a  software organization it features an innovation-targeting culture combined with a specific, custom approach to software development. Software products and components are developed by small teams (SDTs) that are internally diversified by the nationality of individuals, native culture of their organizations and other differences. In addition, the teams are largely self-organizaing, with a large extent of freedom in defining specific processes, or adapting it to the team's needs. Such high diversity creates a friendly ground for innovations on one hand, but also poses a risk for business-driven constraints, effective coordination of work and managing the outcomes.


% present a recap of the old part, i.e. about GEANT teams, BPs etc,
\noindent G\'{E}ANT software teams work in a specific environment that strongly affects the way they work. To a large extent, it results from a federated structure of the organisation and the emphasis put on producing innovation by designing and developing prototypical applications based on the high-performance network, to support novel services for European researchers and citizens~\cite{Stanisavljevic2018}.

Teams in G\'{E}ANT share a common Product Life-cycle (PLC) and use common tools, but they can freely choose and customize their processes and techniques. Team members usually come from various national organizations (called NRENs), can be simultaneously involved in several projects, are geographically distributed, and have diverse cultural and professional backgrounds. This adds an additional complexity that needs to be addressed and embraced.

In response to that, work on Common Best Practices (CBPs)\footnote[1]{\url{https://wiki.geant.org/display/GSD/Catalogue+of+best+practices}} and G\'{E}ANT Software Maturity Model (SMM)\footnote[2]{\url{https://wiki.geant.org/display/GSD/Software+Maturity+Model}} has started in 2018. The preliminary versions of both frameworks have been reviewed by selected software teams, which resulted in revisions that are currently implemented in practice~\cite{Stanisavljevic2018,Walter2020euro}.

The CBPs for G\'{E}ANT software teams provide directional guidance and recommendations on how to achieve specific goals defined in the SMM~\cite{eurospi2019}, but they need to be customized and adapted by the teams to the local context. As a result, the generality of recommendations included in a practice appears to be a balanced trade-off between delivering actionable procedures on one hand and ensuring the necessary generality on the other~\cite{Walter2020euro}. 
A catalogue of Software Best Practices presented in Table~\ref{tab:cbp} covers all relevant aspects of software development that have been identified in G\'{E}ANT in response to the recognized needs and objectives~\cite{Wolski2017} and is one of the tools contributing to software governance. Currently, it includes 24 practices, and a few more are waiting for inclusion into the catalogue. The software governance team (SwM), formed as a part of one of G\'{E}ANT work packages, supports the teams in implementing and adjusting best practices. It also encourages them to share their experience and observations with other teams, creating a continuous improvement loop.

\begin{table}[ht]
\caption{Catalogue of Common Best Practices used in G\'{E}ANT. A--Requirements, B--Design \& implementation, C--Quality assurance, D--Team organization, E--Maintenance}
\begin{tabularx}{\linewidth}{p{0.1\linewidth} p{0.9\linewidth}}
\toprule
ID      & Practice                                                                    \\ 
\midrule
BP-A.1  & Identify an initial group of stakeholders and iteratively refine it \\
BP-A.2  & Elaborate a communication strategy for stakeholders                 \\
BP-A.3  & Identify, analyse and manage requirements                           \\
\midrule
BP-B.1  & Monitor and assess available technologies                           \\
BP-B.2  & Elaborate an approach for documenting processes and artifacts       \\
BP-B.3  & Track the changes in relevant artifacts                             \\
BP-B.4  & Support the build and delivery process with automation                  \\
BP-B.5  & Record and manage issues encountered with the product               \\
BP-B.6  & Verify licenses of the used libraries                               \\
\midrule
BP-C.1  & Identify and manage risk factors that could negatively affect the product \\
BP-C.2  & Identify relevant quality characteristics and test conditions and provide verification criteria for them \\
BP-C.3  & Elaborate and maintain a quality plan for the project               \\
BP-C.4  & Apply adequate methods to verify the outcome of development activities  \\
BP-C.5  & Monitor relevant quality parameters                                 \\
BP-C.6  & Periodically validate the product with project stakeholders         \\
BP-C.7  & Refine the quality assurance process based on retrospection         \\
\midrule
BP-D.1  & Manage skills of the team members and skills required in the project \\
BP-D.2  & Provide effective, adequate and reliable means for communication within the team \\
BP-D.3  & Define and implement an effective decision-making process           \\
BP-D.4  & Manage the schedules and assignments of the team members            \\
\midrule
BP-E.1  & Plan early and implement adequate maintainability-related activities  \\
BP-E.2  & Elaborate a strategy for managing maintenance issues                \\
BP-E.3  & Identify and evaluate available options for implementing a change request \\
BP-E.4  & Define a procedure for deploying changes to running services \\ 
\bottomrule
\end{tabularx}
\label{tab:cbp}
\end{table}

% present the state where we are now
%\footnote{\url{Wolski, M., Walter, B., Marović, B., Todosijević, A., Garnizov, I., Labedzki, M., Mazurek, C., & Rodwell, T. (2020). Deliverable D9 . 2 Software Policy : Common Practices for GN4-3 Software.}} that has been implemented into practice~\cite{Stanisavljevic2018}. 
%The catalogue of CBPss, which addresses the objectives identified in SMM, %\footnote{The catalogue is publicly unavailable}
%\url{https://wiki.geant.org/display/GSD/Catalogue+of+best+practices}}

% present the context of the monitoring and usage

%IVAN - please elaborate with a few sentences about the PLM, and our view on the combination of PLM and BP



%OLD
% GEANT, its structure, objectives and modus operandi - with references to previous papers.

% SMM and CBP - reference to previous paper presenting the practices
% we can again reiterate the challenges GEANT faces: diversity, multi-nationality, multi-cultured, part-time involvement, high level of freedom and independence. Teams cannot be managed, but rather coordinated

%G\'{E}ANT is a pan-European project focused on the development and maintenance of e-infrastructure and services for the research and education community. It operates the backbone network and associated services interconnecting national research and education networks (NRENs) across Europe and enables their collaboration. Also, it is a distributed, innovation-oriented organisation involving participants from many countries and organisations that develop and maintain network-based products and services, frequently based on dedicated or customized software. G\'{E}ANT portfolio comprises currently 30 software projects: some are used directly by G\'{E}ANT; some more are shared or used by NRENs; yet, others contribute to wider open-source communities. 

%A previous analysis of the G\'{E}ANT software development practices

%The motivation for the establishment of a software maturity model for G\'{E}ANT was to determine properly the improvements schema for software teams. Moreover, the practical appliance of maturity model would align the improvement effort with governance frameworks, commonly approved models, and with industry practices. The apparent attractiveness and popularity of the maturity model in the management of the software process and, more broadly, IT management, has contributed to our effort to develop a maturity model specifically for software process improvement (SPI) within G\'{E}ANT, while respecting the seven suggested requirements for the development of maturity models~\cite{Becker2009}.

%The G\'{E}ANT Software Maturity Model (GSMM) has been designed to achieve two primary goals: (1) to capture key practices that already help the teams to successfully deliver software, and (2) to identify areas for further improvements that could be applied by the teams~\cite{eurospi2019,Stanisavljevic2018}.

%The extracted practices can then be shared, adapted and applied by the teams to streamline and align software development processes and governance. The leading factors considered include the lasting nature of G\'{E}ANT, its products and services, distributed nature of conducted collaborations and the existence of many practices that have been established for some time. 

%The resulting model consists of categorised software engineering topics and processes into five key thematic areas, referred to as target areas (TA), namely: requirements engineering; design and implementation; software maintenance; quality assurance; and team organisation. These target areas were elaborated by providing specific content to the maturity model, with each one consisting of several specific goals (SGs) that capture sub-objectives and related activities.


%The GSMM, presented in Sec.~\ref{sec:process}, identifies the core areas and goals that contribute to the effective software development in G\'{E}ANT. However, software teams need not only the targets but also the guidance on how to organise the efforts towards meeting these them, considering the specific context of the organisation. To address this, we created a catalogue of Common Best Practices (CBPs). They have been identified based on three sources of information:
%\begin{itemize}
%%    \item practices currently applied by the software development teams, extracted during the questionnaire interviews (see Sec.~\ref{sec:process}),
%    \item recommendations provided in the literature and case studies concerning similar process optimisation efforts,
%    \item direct or indirect observations made by the software management team.
%\end{itemize}

%The catalogue includes recommendations showing how the particular GSMM specific goals could be addressed, considering the constraints and opportunities present in G\'{E}ANT. Therefore, the best practices balance between the need for providing detailed operational guidance and giving a general direction. Both of these are extremes that would result in missing the objective of providing the teams with effective guidance that they could adapt and implement in their own practice.

%\subsection{Template of a Best Practice}
%\label{ssec:template}

%Description of a best practice includes a large volume of diversified information of various nature and format, which can hinder its readability. To make the practices more accessible for the team members and, consequently, facilitate the adoption of practices, we decided to define a template which presents the data in a structured way. Each practice is presented as a set of attributes that describe key elements of the practice. The template comprises the following attributes:
%\begin{itemize}
%    \item \textbf{Objective} that the practice is expected to address;
%    \item \textbf{Applicability}, describing types of projects or their phases, in which the practice could be effectively applied;
%    \item \textbf{Context} that captures a specific setting (a set of technical, managerial or organisational constraints), for which the practice was identified and for which it is recommended; The practice can be used in other settings, but it may require additional validation;
%    \item \textbf{Addressed elements in GSMM}, linking the practice with the SGs in the GSMM;
%1:1, which means that a single SG is related to a single practice; it could change as a result of the development of other best practices or identification of alternative approaches;
%n:1, where several closely related goals can be simultaneously addressed by a single practice;
%1:n, which captures several best practices that could be used to meet a single SG; the choice of a specific practice depends usually on the specific context. 
%    \item \textbf{Prerequisites}, listing the condition necessary to apply the specific practice;
%    \item \textbf{Recommendation}, outlining actions that should be undertaken to meet the SG; It includes high-level directional advice on \emph{what} to do, with lower-level details on \emph{how} to reach the goal. 
%    \item \textbf{Risks}, describing possible risk factors and their consequences in case of misusing the practice;
%    \item \textbf{Related practices}, indicating other practices that could be applied in a similar context;
%    \item \textbf{Origin}, providing details on how the practice originated.
%\end{itemize}


%The recommendations do not provide direct instructions for the teams on how to proceed in a step-by-step manner, but rather give directional guidance. It includes advice concerning the factors and issues that facilitate addressing the respective goal in the GSMM and that should be considered by the team. As a result, the recommendations presented in a practice are a trade-off between the desire to deliver actionable procedures on one hand and the necessary abstractness on the other. The software teams are expected to analyse and adapt the recommendations to their local context.

%The risk factors capture possible consequences of applying the practice improperly. In this case, they are mostly related to issues of stakeholders identification and management, including prioritisation and identification of relationships among them.

%This specific practice is closely related to the process of defining the communication policy and maintaining contact with stakeholders. These two practices should be used together to ensure the maximum benefit from their implementation.

%The entire catalogue is available for the G\'{E}ANT staff and currently includes 24 practices divided into five target areas that directly correspond to areas in the GSMM. Each practice addresses one or more SGs defined in the GSMM and, currently, all the goals are covered.


